General Equilibrium Theory for Climate Change

We propose two general equilibrium models, quota equilibrium and emission tax equilibrium. The government specifies quotas or taxes on emissions, then refrains from further action. Quota equilibrium exists; the allocation of emission property rights strongly impacts the distribution of welfare. If the only externality arises from total net emissions, quota equilibrium is constrained Pareto Optimal. Every quota equilibrium can be realized as an emission tax equilibrium and vice versa. However, for certain tax rates, emission tax equilibrium may not exist, or may exhibit high multiplicity. Full Pareto Optimality of quota equilibrium can often be achieved by setting the right quota.

==> myvruler.tex <==
\usepackage{vruler}
\setvruler[10pt][1][1][4][1][20pt][20pt][0pt][\textheight]
\let\orgfillzeros\fillzeros
\def\fillzeros[#1]#2{%
  \begingroup
    \color[rgb]{0.8,0.8,0.8}%
    \orgfillzeros[{#1}]{#2}%
  \endgroup
}


==> novruler.tex <==
% nothing here


==> prodabstract.tex <==
This paper presents a general equilibrium model with infinitely many agents, individualistic consumption externalities and bads. We identify and resolve critical flaws of general equilibrium theory (GE) that are specific to the presence of bads such as free-disposal in production and failure of uniform integrability, and show that the model is coherent (i.e equilibrium exists), hence addressing the question raised in \citet{ha05}. 
The main technical drive of the paper is nonstandard analysis, which allows us to (1) construct the so-called Loeb space which has a richer measure theoretic structure compare with standard measure spaces; (2) import results that are true in finite GE models to results in GE models with infinitely many agents. We give examples that illustrate generality and applicability of the result. 
